Polynomial-Time Algorithms for Multi-Agent Minimal-Capacity Planning

We study the problem of minimizing the resource capacity of autonomous agents cooperating to achieve a shared task. More specifically, we consider high-level planning for a team of homogeneous agents that operate under resource constraints in stochastic environments and share a common goal: given a set of target locations, ensure that each location will be visited infinitely often by some agent almost surely. We formalize the dynamics of agents by consumption Markov decision processes. In a consumption Markov decision process, the agent has a resource of limited capacity. Each action of the agent may consume some amount of the resource. To avoid exhaustion, the agent can replenish its resource to full capacity in designated reload states. The resource capacity restricts the capabilities of the agent. The objective is to assign target locations to agents, and each agent is only responsible for visiting the assigned subset of target locations repeatedly. Moreover, the assignment must ensure that the agents can carry out their tasks with minimal resource capacity. We reduce the problem of finding target assignments for a team of agents with the lowest possible capacity to an equivalent graph-theoretical problem. We develop an algorithm that solves this graph problem in time that is \emph{polynomial} in the number of agents, target locations, and size of the consumption Markov decision process. We demonstrate the applicability and scalability of the algorithm in a scenario where hundreds of unmanned underwater vehicles monitor hundreds of locations in environments with stochastic ocean currents.

==> number_of_targets2.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
width=6.5cm,
grid=both,
x grid style={white!69.0196078431373!black},
xlabel={\large Number of Agents},
legend style={font=\normalsize},
xmin=0.5, xmax=209.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-0.214715121219719, ymax=4.57622144516709,
ytick style={color=black}
]
\path [draw=color0, thick]
(axis cs:10,0.0159535201169696)
--(axis cs:10,0.0388692347429547);

\path [draw=color0, thick]
(axis cs:20,0.0263994863318031)
--(axis cs:20,0.0431729147149498);

\path [draw=color0, thick]
(axis cs:30,0.0225950191165227)
--(axis cs:30,0.0359035780285579);

\path [draw=color0, thick]
(axis cs:40,0.0177848662197543)
--(axis cs:40,0.0335802231967496);

\path [draw=color0, thick]
(axis cs:50,0.0194917720093616)
--(axis cs:50,0.0341647583708874);

\path [draw=color0, thick]
(axis cs:60,0.0153023471345826)
--(axis cs:60,0.0378558168897704);

\path [draw=color0, thick]
(axis cs:70,0.00962207371902851)
--(axis cs:70,0.0518045658378563);

\path [draw=color0, thick]
(axis cs:80,0.0163088915722142)
--(axis cs:80,0.0369291903598537);

\path [draw=color0, thick]
(axis cs:90,0.0157430626150408)
--(axis cs:90,0.0320755742791853);

\path [draw=color0, thick]
(axis cs:100,0.0109094303624297)
--(axis cs:100,0.0297238189204072);

\path [draw=color0, thick]
(axis cs:110,0.0133279664927258)
--(axis cs:110,0.0312533752507434);

\path [draw=color0, thick]
(axis cs:120,0.0100889502294153)
--(axis cs:120,0.02284156696724);

\path [draw=color0, thick]
(axis cs:130,0.00638385146889127)
--(axis cs:130,0.0313145604726371);

\path [draw=color0, thick]
(axis cs:140,0.00305472270695436)
--(axis cs:140,0.0374541436031653);

\path [draw=color0, thick]
(axis cs:150,0.00892149279628977)
--(axis cs:150,0.0245956533142449);

\path [draw=color0, thick]
(axis cs:160,0.0070390819026977)
--(axis cs:160,0.0213003994510621);

\path [draw=color0, thick]
(axis cs:170,0.0103999566607391)
--(axis cs:170,0.0237803507275666);

\path [draw=color0, thick]
(axis cs:180,0.0109523466774646)
--(axis cs:180,0.0248676368048962);

\path [draw=color0, thick]
(axis cs:190,0.0111355656305921)
--(axis cs:190,0.0237124806722033);

\path [draw=color0, thick]
(axis cs:200,0.00875240800716785)
--(axis cs:200,0.0304655647482643);

\path [draw=color1, thick]
(axis cs:10,0.0152245165215221)
--(axis cs:10,0.0221378682746205);

\path [draw=color1, thick]
(axis cs:20,0.0654820769699976)
--(axis cs:20,0.0988204390135839);

\path [draw=color1, thick]
(axis cs:30,0.11336347155284)
--(axis cs:30,0.158101567700395);

\path [draw=color1, thick]
(axis cs:40,0.168803633153639)
--(axis cs:40,0.242854582369127);

\path [draw=color1, thick]
(axis cs:50,0.300741833288206)
--(axis cs:50,0.40052021161841);

\path [draw=color1, thick]
(axis cs:60,0.400144310204212)
--(axis cs:60,0.493046622069652);

\path [draw=color1, thick]
(axis cs:70,0.52841224141322)
--(axis cs:70,0.857950811908618);

\path [draw=color1, thick]
(axis cs:80,0.688079659665123)
--(axis cs:80,0.972749121462806);

\path [draw=color1, thick]
(axis cs:90,0.869094477393521)
--(axis cs:90,1.17275976111661);

\path [draw=color1, thick]
(axis cs:100,0.861767770424726)
--(axis cs:100,1.51866147361672);

\path [draw=color1, thick]
(axis cs:110,1.28109423576507)
--(axis cs:110,1.72446671069947);

\path [draw=color1, thick]
(axis cs:120,1.37533267784801)
--(axis cs:120,1.84755037974629);

\path [draw=color1, thick]
(axis cs:130,1.58546289936469)
--(axis cs:130,2.01103723510338);

\path [draw=color1, thick]
(axis cs:140,1.95941633598098)
--(axis cs:140,2.18696785553208);

\path [draw=color1, thick]
(axis cs:150,2.24421365324462)
--(axis cs:150,2.61028432782686);

\path [draw=color1, thick]
(axis cs:160,1.65256602107542)
--(axis cs:160,3.33484144867403);

\path [draw=color1, thick]
(axis cs:170,2.89056477858647)
--(axis cs:170,3.26589176342861);

\path [draw=color1, thick]
(axis cs:180,2.56289591834059)
--(axis cs:180,4.12072982743273);

\path [draw=color1, thick]
(axis cs:190,3.60241528287128)
--(axis cs:190,3.99176017508313);

\path [draw=color1, thick]
(axis cs:200,4.01436274907747)
--(axis cs:200,4.3365181598886);

\path [draw=color2, thick]
(axis cs:10,0.0326760593679192)
--(axis cs:10,0.0595090802881477);

\path [draw=color2, thick]
(axis cs:20,0.0925471513987334)
--(axis cs:20,0.141327765631601);

\path [draw=color2, thick]
(axis cs:30,0.137332114400341)
--(axis cs:30,0.192631521997975);

\path [draw=color2, thick]
(axis cs:40,0.189801345320239)
--(axis cs:40,0.273221959619031);

\path [draw=color2, thick]
(axis cs:50,0.32214853975988)
--(axis cs:50,0.432770035526986);

\path [draw=color2, thick]
(axis cs:60,0.420365009393788)
--(axis cs:60,0.52598408690443);

\path [draw=color2, thick]
(axis cs:70,0.547254530755622)
--(axis cs:70,0.900535162123101);

\path [draw=color2, thick]
(axis cs:80,0.705750503542902)
--(axis cs:80,1.0083163595171);

\path [draw=color2, thick]
(axis cs:90,0.887649650534921)
--(axis cs:90,1.20202322486944);

\path [draw=color2, thick]
(axis cs:100,0.874866607445938)
--(axis cs:100,1.54619588587834);

\path [draw=color2, thick]
(axis cs:110,1.29848473731194)
--(axis cs:110,1.75165755089607);

\path [draw=color2, thick]
(axis cs:120,1.38802945212657)
--(axis cs:120,1.86778412266438);

\path [draw=color2, thick]
(axis cs:130,1.59897112839329)
--(axis cs:130,2.03522741801632);

\path [draw=color2, thick]
(axis cs:140,1.97216676611654)
--(axis cs:140,2.21472629170664);

\path [draw=color2, thick]
(axis cs:150,2.25351138916812)
--(axis cs:150,2.63450373801389);

\path [draw=color2, thick]
(axis cs:160,1.66133468158759)
--(axis cs:160,3.35441226951562);

\path [draw=color2, thick]
(axis cs:170,2.90142744653012)
--(axis cs:170,3.28920940287326);

\path [draw=color2, thick]
(axis cs:180,3.57587117435281)
--(axis cs:180,4.14357455490287);

\path [draw=color2, thick]
(axis cs:190,3.6143137116843)
--(axis cs:190,4.0147097925729);

\path [draw=color2, thick]
(axis cs:200,4.03164728048108)
--(axis cs:200,4.35845160124041);

\addplot [thick, color0, mark=*, mark size=3, mark options={solid}]
table {%
10 0.0274113774299622
20 0.0347862005233765
30 0.0292492985725403
40 0.025682544708252
50 0.0268282651901245
60 0.0265790820121765
70 0.0307133197784424
80 0.0266190409660339
90 0.023909318447113
100 0.0203166246414185
110 0.0222906708717346
120 0.0164652585983276
130 0.0188492059707642
140 0.0202544331550598
150 0.0167585730552673
160 0.0141697406768799
170 0.0170901536941528
180 0.0179099917411804
190 0.0174240231513977
200 0.0196089863777161
};
\addlegendentry{Bottleneck time}
\addplot [thick, color1, mark=*, mark size=3, mark options={solid}]
table {%
10 0.0186811923980713
20 0.0821512579917908
30 0.135732519626617
40 0.205829107761383
50 0.350631022453308
60 0.446595466136932
70 0.693181526660919
80 0.830414390563965
90 1.02092711925507
100 1.19021462202072
110 1.50278047323227
120 1.61144152879715
130 1.79825006723404
140 2.07319209575653
150 2.42724899053574
160 2.49370373487473
170 3.07822827100754
180 3.34181287288666
190 3.7970877289772
200 4.17544045448303
};
\addlegendentry{SCC time}
\addplot [thick, color2, mark=*, mark size=3, mark options={solid}]
table {%
10 0.0460925698280334
20 0.116937458515167
30 0.164981818199158
40 0.231511652469635
50 0.377459287643433
60 0.473174548149109
70 0.723894846439362
80 0.857033431529999
90 1.04483643770218
100 1.21053124666214
110 1.525071144104
120 1.62790678739548
130 1.8170992732048
140 2.09344652891159
150 2.444007563591
160 2.50787347555161
170 3.09531842470169
180 3.35972286462784
190 3.8145117521286
200 4.19504944086075
};
\addlegendentry{Total time}
\end{axis}

\end{tikzpicture}


==> tikzlibrarycmdps.code.tex <==
%oo\tikzstyle{target}=[fill=blue!15]
%\tikzstyle{reload}=[accepting]

\tikzset{state/.append style={fill=blue!4}}
\tikzstyle{target}=[fill=green!70!black!25]
\tikzstyle{reload}=[accepting]

% Probability labels
\tikzstyle{prob}=[
  color=black!50,
  outer sep=-2pt,
  pos=.8,
]

% Consumption labels
\tikzstyle{cons} = [
  execute at begin node = {$[$},%
  execute at end node = {$]$},
  outer sep=0pt,
  pos=.5,
]

\tikzstyle{shifted below} = [
  below,  outer sep=15pt,
]

% Value boxes
\tikzstyle{valbox} = [
  rounded corners=2pt,
  shifted below,
  inner sep=.5pt,
  draw,
  font=\footnotesize,
  minimum size=1em,
]

\tikzset{
  objective/.style = {
    label={[label position=north, anchor=south, below,
    xshift=0pt, yshift=-4pt,
    fill=white, scale=.5,
    draw, rounded corners=1pt, very thin]#1}
  },
  obj prob/.style = {
    label={[label position=south, anchor=north, above,
    xshift=0pt, yshift=4pt,
    fill=white, scale=.5,
    draw, rounded corners=1pt, very thin]#1}
  },
  nonreloading/.style = {
    objective=$\nonreloading$,
    fill=orange!15,
  },
  safety/.style = {
    objective=$\safety$,
    fill=blue!15,
  },
  pos reach/.style = {
    objective=$\reachability$,
    obj prob=${}>0$,
    fill=green!70!black!20,
  },
  as reach/.style = {
    objective=$\reachability$,
    obj prob=$\as$,
    fill=green!70!black!20,
  }
}

\tikzstyle{capacity} = [
  rounded corners,
  draw,
  fill=yellow!40,
]

==> tikzlibrarygridworld.code.tex <==
\usepackage{xcolor}

\usetikzlibrary{arrows.meta}

\definecolor{background}{rgb}{0.85,1.0,1.0}
\definecolor{agent}{rgb}{0.42,0.42,0.42}

\tikzstyle{action edge} = [thick,shorten >=1pt,>={Stealth[round]}]
\tikzstyle{side effect} = [gray, shorten >=4pt, looseness=\loose, green!60!black!40]
\tikzstyle{main} = [shorten >=-4pt, very thick, green!60!black]

\tikzstyle{cell} = [minimum size=\step, xshift=.1255cm, yshift=.1245cm, transform shape]

\tikzstyle{agent} = [minimum size=15pt, rounded corners, draw=agent,fill=agent]
\tikzstyle{action name} = [font={\scriptsize\sffamily}, align=center, scale=.7]
\tikzstyle{gridworld} = [gray, ultra thin]

\tikzstyle{reload} = []

\def\loose{.7}

==> tikzlibrarymyautomata.code.tex <==
% Automata stuff
\usetikzlibrary{automata}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{bending}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}
\usetikzlibrary{shapes}

\def\accsize{6pt}

\tikzset{
  >={Stealth[round,bend]},
}

\tikzstyle{automaton}=[
  % Use nice arrows that do not touch their destination.
  semithick,shorten >=1pt,>={Stealth[round,bend]},
  % Encourage a common distance between all states.
  node distance=1.7cm,
  % Disable the "start" text in front of the initial arrow.
  initial text=,
  % Allows to use scale to scale the figure
%  transform shape,
  % Reduce the size of the hidden node at the beginning of the initial arrow.
  every initial by arrow/.style={every node/.style={inner sep=0pt}},
  % Encourage a common size of all states that is smaller than the default.
  every state/.style={
    align=center,
    fill=white,
    minimum size=6mm,
    inner sep=0pt,
  },%
]

\tikzstyle{smallautomaton}=[
  automaton,
  node distance=8mm,
  every state/.style={minimum size=4mm,fill=white,inner sep=1pt}
]

\tikzstyle{mediumautomaton}=[
  automaton,
  node distance=1cm,
  every state/.style={minimum size=5mm,fill=white,inner sep=2pt}
]

\tikzstyle{cstate}=[state,rounded rectangle,text width=,]

% This is used for runs vizualization
\tikzstyle{dot}=[fill=black,circle,minimum size=4pt,inner sep=0]

\makeatletter
\tikzoption{initial angle}{\tikzaddafternodepathoption{\def\tikz@initial@angle{#1}}}
\makeatother

% pass "initial overlay" as a parameter to the tikz figure if you want
% to initial arrow to be ignored from the computation of the figure
% box.  This might be needed for better caption centering.
\tikzstyle{initial overlay}=[every initial by arrow/.append style={overlay}]

\tikzstyle{unreachable} = [densely dotted]

% % % Usage: \node[acclabel]{label\strut}
% The command \strut makes all labels have the same height.
\tikzstyle{acclabel} = [
  fill=yellow!20,
  rounded corners=3pt,
  draw=black,
  inner ysep=0pt,
  inner xsep=3pt,
]
\tikzstyle{ltllabel} = [acclabel,fill=darkgreen!20]

\tikzstyle{namelabel} = [
  execute at begin node = {$($},%
  execute at end node = {$)$}
]

\tikzstyle{matrix of states} = [
matrix of nodes,
every node/.style={state},
column sep=.8cm,
row sep=.8cm,
execute at empty cell={
  \node[transparent,name=
    \tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]{};]},
]

% Acceptance sets are displayed as small circles with white
% sans-serif number.  The default color is light blue. Can be
% changed by collacc styles.  Use anchor=center to ignore the
% predefined anchor on edges like "loop above" or "loop left"
% or when using path[auto].
\tikzstyle{accset}=[
  circle,inner sep=.9pt,
  draw=none, %draw=white,
  solid,
  collacc0, text=white,
  thin,
  anchor=center,
  font=\bfseries\tiny, %\sffamily
  minimum size={\accsize},
]
% Acceptance set as square
\tikzstyle{accsquare}=[accset,rectangle,inner sep=1.9pt,rounded corners=0pt]

% % % Colors % % %
\tikzset{
  collacc0/.style={fill=blue!50!cyan},
  collacc1/.style={fill=orange!90!black},
  collacc2/.style={fill=green!70!black},
  collacc3/.style={fill=red!80!black},
  collacc4/.style={fill=magenta},
  collacc5/.style={fill=blue!50!black},
}


% The key /sacc/where is used to determine where the acc marks on
% states should be placed using the sacc/derived keys
% The default value is center
% It has to be used in scopes, does not work inside nodes
\pgfkeyssetvalue{/sacc/where}{center}
\tikzset{
  sacc where/.code={
    \pgfkeyssetvalue{/sacc/where}{#1}
  }
}

% % % Labels and marks of automata % % %
\tikzset{
  % Labels of edges that have some acceptance mark. Shifts label
  % further from the edge to avoid ugly clash with the mark.
  % Usage:
  %   (n1) edge pic[pos=.3,left]{l=LABEL}
  l/.pic={\node[outer sep=3pt] {#1};},%
  % A colored mark with number inside. Use acc for a small circle and
  % accsq for a small square.
  % Usage:
  %   (n1) edge pic[pos=.3]{acc=ACC_ID}
  % collaccACC_ID must be defined
  acc/.pic={\node[accset,collacc#1]{#1};},%
  accsq/.pic={\node[accsquare,collacc#1]{#1};},%
  % No number inside the bullets
  eacc/.pic={\node[accset,collacc#1]{\emptyacc};},%
  eaccsq/.pic={\node[accsquare,collacc#1]{\emptyacc};},%
  % State labels on north east
  sacc/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {acc=#1}}
  },
  saccsq/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {accsq=#1}}
  },
  esacc/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eacc=#1}}
  },
%  esacc/.style 2 args = {
%    append after command=
%      {pic[#2] at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eacc=#1}}
%  },
  esaccsq/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eaccsq=#1}}
  },
  % Easy typesetting of colored accepting marks with custom labels.
  % Usage:
  %   (n1) edge pic[pos=.3]{acc={COLOR_ID}{LABEL}}
  % collaccCOLOR_ID must be defined
  pics/cacc/.style 2 args={%
    code={\node[accset,collacc#1]{#2};}%
  },%
  pics/caccsq/.style 2 args={%
      code={\node[accsquare,collacc#1]{#2};}%
    },%
  csacc/.style 2 args = {%
      append after command=%
        {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {cacc={#1}{#2}}}%
  },%
  csaccsq/.style 2 args = {%
      append after command=%
        {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {caccsq={#1}{#2}}}%
  },%
}

% Macros for colored acceptance marks used in text. Usage:
% \tacc{COLOR_ID}{LABEL}
\def\markbaseline{-.37em}
\def\tacc#1{\tikz[baseline=\markbaseline]\pic{acc=#1};\xspace}
\def\tcacc#1#2{\tikz[baseline=\markbaseline]\pic{cacc={#1}{#2}};\xspace}
\def\taccsq#1{\tikz[baseline=\markbaseline]\pic{accsq=#1};\xspace}
\def\tcaccsq#1#2{\tikz[baseline=\markbaseline]\pic{caccsq={#1}{#2}};\xspace}

% % % some predefined marks with no number inside
\def\emptyacc{\phantom{0}}
\def\gm{\tcacc{2}{\emptyacc}}
\def\om{\tcacc{1}{\emptyacc}}
\def\bm{\tcacc{0}{\emptyacc}}
\def\bsq{\tcaccsq{0}{\emptyacc}}
\def\rsq{\tcaccsq{3}{\emptyacc}}

\def\minimark#1{
\def\emptyacc{}
\def\accsize{4pt}
#1
}

